Predictive Software Measures based on Z Specifications - A Case Study

Estimating the effort and quality of a system is a critical step at the beginning of every software project. It is necessary to have reliable ways of calculating these measures, and, it is even better when the calculation can be done as early as possible in the development life-cycle. Having this in mind, metrics for formal specifications are examined with a view to correlations to complexity and quality-based code measures. A case study, based on a Z specification and its implementation in ADA, analyzes the practicability of these metrics as predictors.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{C. Andr\'es and L. Llana (Eds.): 2nd Workshop on Formal\\
Methods in the Development of Software 2012 (WS-FMDS 2012).\\
EPTCS 86, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.86.5}{10.4204/EPTCS.86.5}}

